Recommending Code Understandability Improvements based on Code Reviews

Developers spend 70% of their time understanding code. Code that is easy to read can save time, while hard-to-read code can lead to the introduction of bugs. However, it is difficult to establish what makes code more understandable. Although there are guides and directives on improving code understandability, in some contexts, these practices can have a detrimental effect. Practical software development projects often employ code review to improve code quality, including understandability. Reviewers are often senior developers who have contributed extensively to projects and have an in-depth understanding of the impacts of different solutions on code understandability. This paper is an early research proposal to recommend code understandability improvements based on code reviewer knowledge. The core of the proposal comprises a dataset of code understandability improvements extracted from code reviews. This dataset will serve as a basis to train machine learning systems to recommend understandability improvements.

==> unused_text.tex <==
%Define which code alternatives (i.e., code snippet differents but functionally equivalents) are easier to read than another one is challenging, and researchers have performed some experiments. For example, Miara et al. \cite{Miara1983} and Bauer et al. \cite{Bauer2019} evaluated which indentation level is the best to understandability. Likewise, Gopstein et al. \cite{Gopstein2017, Gopstein2018}, Medeiros et al. \cite{Medeiros2019}, and Santos et al. \cite{dosSantos2018} investigated whether some code patterns (e.g., pre and post-increment, multiple statements per line, and conditional operator) cause misunderstanding or whether they are more readable.


%For example, Gopstein et al. \cite{Gopstein2017} performed an experiment to confirm whether some small code patterns are atoms of confusion, i.e., code patterns that cause misunderstanding while its alternative does not. They asked students to answer the output of code snippets with candidates of atoms of confusion and other code snippets with their alternatives and found 15 atoms of confusion. Similarly, Medeiros et al. \cite{Medeiros2019} asked developers to give their opinion if some of those atoms of confusion (named misunderstanding pattern by Medeiros et al.) influence the code understanding negatively. However, they did not find the same results as Gopstein et al. for some atoms of confusion (e.g., conditional operator and pre-increment) causing uncertainty for these patterns.

%Nevertheless, some studies did not find a statistical difference between alternatives \cite{}. Moreover, among those which found a statistical difference, some contracted previously found results (e.g., \cite{Gopstein2017, Medeiros2019}), and some found a statistical difference in specifics scenarios (e.g., \cite{Bauer2019, Schankin2018, Lawrie2007}). 

%The goal of this work is to recommend code understandability improvements to developers. To this end, we will train a Machine Learning (ML) to translate code hard-to-read into code easy-to-read. Our approach is presented in \autoref{fig:approach} and is divided into the following steps:

%\circled{1} \underline{Dataset of Code Reviews related to Code Understandability}: we will classify manually code reviews of selected projects on GitHub.

%\circled{2} \underline{Dataset of Code Reviews Extended}: we will use our dataset built on step \circled{1} to train an ML to classify more code reviews and expand our dataset.

%\circled{3} \underline{Dataset of Code Understandability Improvements}: using our dataset expanded of step \circled{2}, we will extract the version before (v) and the version after (v+1) code understandability improvement to create a dataset of pairs (v, v+1).

%\circled{4} \underline{Recommendation System to Code Understandability Improvements}: we will use the dataset built on step \circled{3} as input to train an ML to translate code hard-to-read into code easy-to-read.

%GitHub, for example, is a popular tool that integrates the function of MCR in the pull-based model. In that process, developers submit their code changes through pull-requests, and reviewers inspect the code suggesting code repair and improvements through general and inline comments. While general comments are remarks of the whole code changes, the inline comments are directed to a specific code line.


%\section{Related Works}

%Maybe these papers are more related
%Characteristics of Useful Code Reviews: An Empirical Study at Microsoft
%Predicting Usefulness of Code Review Comments Using Textual Features and Developer Experience

%We did not find a dataset of code understandability improvements in the literature, only datasets of code reviews. For example, the dataset created by Zhang et al. \cite{zhang2020} is the most extensive dataset with code reviews data to the best of our knowledge. That dataset contains 96 features collected from 11,230 projects and 3,347,937 pull requests. However, none of those data indicates which code review comments are related to understandability improvement. On the other hand, the dataset by Paixao et al. \cite{paixao2018} is the most similar to what we propose, associate code reviews with code changes. They built a dataset that links code review with the complete version of the code. But, they not classified if the code review is related to understandability improvement.

%\todo{And they tend to overreport, which often leads to them being ignored.}
%We found many tools able to detect and fix rules violations warned by static code analysis tools. For example, the SpongeBugs \cite{marcilio2019automatically} is a rule-based tool that automatically detects and fixes violations of 11 different rules. The downside of rule-based tools is that they are limited to make just code improvements that they were designed. Also, they tend to overreport, which often leads to them being ignored. Alternatively, the Styler \cite{loriot2019} is a machine-learning-based tool to fix Checkstyle formatting rules violations. That tool injects errors in violation-free source code to induces rules violation and generate training data. Therefore, the Style is limited to learning only formatting improvements based on rules violations.

%At present, we are working on the manual classification of code reviews. In that step, our goal is to evaluate if the comments of the reviewer intend to improve understandability. This implies that we need to look beyond the text. For example, we found a comment~\footnote{\url{https://github.com/apache/skywalking/pull/4332\#discussion_r376758126}} "This could be replaced by simplier foreach.", where the reviewer suggests a solution that makes the code simpler. When we look at the code, we realize that the intent is to make the code more verbose and easy to understand. In another context, to simplify is the inverse. In the comment~\footnote{\url{https://github.com/apache/skywalking/pull/4332\#discussion_r376758126}} "true that this expression is equivalent and simpler but less readable. I would prefer a revert", the reviewer suggests that the simple logical expression, that has one less condition, is less readable.
